Benchmarking TPU, GPU, and CPU Platforms for Deep Learning

Training deep learning models is compute-intensive and there is an industry-wide trend towards hardware specialization to improve performance. To systematically benchmark deep learning platforms, we introduce ParaDnn, a parameterized benchmark suite for deep learning that generates end-to-end models for fully connected (FC), convolutional (CNN), and recurrent (RNN) neural networks. Along with six real-world models, we benchmark Google's Cloud TPU v2/v3, NVIDIA's V100 GPU, and an Intel Skylake CPU platform. We take a deep dive into TPU architecture, reveal its bottlenecks, and highlight valuable lessons learned for future specialized system design. We also provide a thorough comparison of the platforms and find that each has unique strengths for some types of models. Finally, we quantify the rapid performance improvements that specialized software stacks provide for the TPU and GPU platforms.

==> background.tex <==
\section{Background?}




==> casestudies.tex <==
\section{System Balance on the TPU Platform}
\label{sec:casestudy}

Previous sections focus on accelerator performance, and the results from DNNSynBench
avoid most host overheads because data is synthesized on the host. In this section, we perform a 
case study of the TPU platform with the real workloads to uncover system design bottlenecks using the TPU performance profiler. This tool collects traces and corresponding statistics.
%This allow us to reinforce knowledge learned from synthetic benchmarks.
%Such profiling is not supported on the GPU. 

By analyzing the TPU bottlenecks of the real workloads, we show the importance of system balance when designing accelerator systems.
We observe that for workloads bound by feeding data to the TPU device, performance can be improved by at least 35\% if the bottleneck is resolved.
We find that RetinaNet and SqueezeNet are bottlenecked by data infeeding, DenseNet and MobileNet by the device, and ResNet-50 is bottlenecked by the device when float32 is used, and slightly by data infeeding with bfloat16. We collect profiling data using TensorFlow 1.9.

The TPU platform is composed of a CPU host and a TPU device.
The architecture is described in the TPU v2 presentation at Hot Chips 2017~\cite{dean2017hotchips}.
Here we refer to anything outside of the device as data infeeding, including the host, the link 
between the host and device, and the network overhead for the host to fetch the raw data.
A workload is bottlenecked if the relative load on data infeeding and the device is not balanced.

For real data, the CPU host fetches images from the network file system, decodes, 
preprocesses, and feeds them to the device. \Fig{fig:casestudy} calls this data preparation.
The device then performs training computation on the images. 
We can also modify the real workloads to use synthetic data to quantify data infeeding time by avoiding data preparation overheads.

Using bfloat16 can improve both data infeed and device computation, because data size is cut in half.
Data infeeding through PCIe can be improved by approximately 2$\times$, since images are 50\% as large and the labels do not change.
The computation in the device can be improved because of bandwidth reduction from HBM to MXU.

%By comparing the performance with different computation capacity and data infeed requirement, we can analyze whether a workload is bottlenecked by host or device.

\Fig{fig:casestudy} shows FLOPS utilization (top) and infeed time (bottom) of the real workloads.
We enumerate the products of \{float32, bfloat16\} and \{with, without data preparation\} for each.
FLOPS utilization measures computation efficiency and infeed time measures how long the device waits for data.
The statistics are collected from the TPU profiler.
The error bars are one standard deviation of the one-minute samples from the profiler.
We see that a workload can be bottlenecked by device or data with different degrees under different circumstances.
%The workload can make the most of the system only when the system is balanced.

\begin{figure}[t]
\begin{center}
\includegraphics[width=.9\columnwidth]{casestudy/flops_infeed.pdf}
\caption{FLOPS utilization (top) and infeed time (bottom) of the real workloads using float32 and bfloat16, with and without data preparation. Models with large infeed time percentage, RetinaNet and SqueezeNet, are limited by data infeed.}
\label{fig:casestudy}
\vspace{-1em}
\end{center}
\end{figure}

RetinaNet and SqueezeNet are bottlenecked by data infeed, as the performance increases by using synthetic data as seen
in \Fig{fig:casestudy}. 
After eliminating the data infeed bottleneck, the performance improvement is 35\% for RetinaNet and 129\% for SqueezeNet using bfloat16.
SqueezeNet is the smallest of the real models and the only one with data infeed percentages even when using synthetic data, demonstrating that
the fast TPU computation for model training creates an Amdahl's bottleneck on data infeed. RetinaNet's bottleneck is likely due to the fact 
that it uses the COCO dataset (640x640 images), while others use the ImageNet dataset (224x224 images).
%The data preprocessing of RetinaNet include
%category classification, bounding box regression, and number of
%positive examples to normalize the loss during training.

We see that switching RetinaNet, ResNet-50 and SqueezeNet from float32 to bfloat16 with real data, the data infeed percentage 
increases, together with the FLOPS percentage. This indicates that the performance improvement in the device is larger than 
the reduction in PCIe bandwidth. In contrast, when using synthetic data, the infeed time of SqueezeNet decreases with the 
change from float32 to bfloat16, indicating that the reduction in bandwidth is higher than improvement in the device.

ResNet-50 is bottlenecked by the device when using float32, and slightly by data infeed when using bfloat16.
\Fig{fig:casestudy}(top) shows that switching from float32 to bfloat16 increases performance.
With real data and float32, the bottleneck is mainly on the device, but switching to bfloat16 increases the infeed time from 
0 to 3.2\%. Switching from real data to synthetic data improves the performance by about 22\%.
When bottlenecks are resolved, the estimated performance improvement is 15\%.

DenseNet and MobileNet are bottlenecked by the device.
The performance of both workloads is increased by switching from float32 to bfloat16, using real data.
The use of synthetic data does not affect performance, so the workloads are not limited by data infeed.

